Latent Communication in Artificial Neural Networks

As NNs permeate various scientific and industrial domains, understanding the universality and reusability of their representations becomes crucial. At their core, these networks create intermediate neural representations, indicated as latent spaces, of the input data and subsequently leverage them to perform specific downstream tasks. This dissertation focuses on the universality and reusability of neural representations. Do the latent representations crafted by a NN remain exclusive to a particular trained instance, or can they generalize across models, adapting to factors such as randomness during training, model architecture, or even data domain? This adaptive quality introduces the notion of Latent Communication -- a phenomenon that describes when representations can be unified or reused across neural spaces. A salient observation from our research is the emergence of similarities in latent representations, even when these originate from distinct or seemingly unrelated NNs. By exploiting a partial correspondence between the two data distributions that establishes a semantic link, we found that these representations can either be projected into a universal representation, coined as Relative Representation, or be directly translated from one space to another. Latent Communication allows for a bridge between independently trained NN, irrespective of their training regimen, architecture, or the data modality they were trained on -- as long as the data semantic content stays the same (e.g., images and their captions). This holds true for both generation, classification and retrieval downstream tasks; in supervised, weakly supervised, and unsupervised settings; and spans various data modalities including images, text, audio, and graphs -- showcasing the universality of the Latent Communication phenomenon. [...]

==> config/preamble.tex <==
\usepackage{overpic}
\usepackage{multirow}
% \usepackage[marginpar]{todo}
\usepackage{todo}

% \usepackage{lmodern}
\usepackage{mathpazo} % Use the Palatino font by default

% Needed if not using the xelatex LaTeX engine
\usepackage[utf8]{inputenc} % Required for inputting international characters
\usepackage[T1]{fontenc} % Output font encoding for international characters

\usepackage[autostyle=true]{csquotes} % Required to generate language-dependent quotes in the bibliography

% Required for good position of the footnote
% https://tex.stackexchange.com/questions/4902/why-is-my-footnote-glued-to-the-text
\usepackage[bottom]{footmisc}


\usepackage{soul}
\usepackage{wrapfig}
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{xcolor} % Required for specifying custom colours
\usepackage{colortbl} % Required for colouring tables
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% Use \mathscr for lowercase mathcal
\usepackage[scr=boondoxo, scrscaled=1.05]{mathalpha}


\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{tikz-3dplot}
\pgfplotsset{compat=1.16}


%----------------------------------------------------------------------------------------
%	COLOURS
%----------------------------------------------------------------------------------------
% Needs to be here because must be loaded at the start of the class

% Main Colors
\definecolor{sapienzared}{RGB}{130,36,51}
\definecolor{highlight}{HTML}{D2691E} %Orange: {E36414}
\colorlet{subtitlecolor}{darkgray}
% \colorlet{mdtRed}{red!50!black}

% Contents color
\definecolor{pltorange}{rgb}{1.        , 0.49803922, 0.05490196}
\definecolor{pltblue}{rgb}{0.12156863, 0.46666667, 0.70588235}

\definecolor{colorxstuff}{HTML}{7B113A}
\definecolor{colorystuff}{HTML}{4F6F52}

% Subtitle


==> config/styling.tex <==
%-------------------------------------------------------------------------------
%    CHAPTER WITH SUBTITLE
%-------------------------------------------------------------------------------

\newcommand\Chapter[2]{
  \chapter[#1]{#1\\\color{subtitlecolor}\medskip\large\itshape#2}
}


%----------------------------------------------------------------------------------------
%	GLOSSARIES
%----------------------------------------------------------------------------------------
\usepackage[automake,symbols,abbreviations,nomain,nogroupskip]{glossaries-extra}
\makeglossaries
\setabbreviationstyle[withoutdesc]{short-long}
\setabbreviationstyle[withdesc]{short-long-desc}
\setabbreviationstyle[nolong]{short-nolong}

\input{glossaries/symbols}
\input{glossaries/abbreviations}

%-------------------------------------------------------------------------------
%                Bibliography
%-------------------------------------------------------------------------------
% Use the bibtex backend with the authoryear citation style (which resembles APA)

% http://www.hansenlab.org/cv_bibliography_tex
\usepackage[
  backend=biber,
  bibstyle=alphabetic,
  style=authoryear,
  sorting=ydnt,
  sortcites=true,
  natbib=true,
  % defernumbers=true,
  maxbibnames=99,
  giveninits=false,
  uniquename=init,
  url=true,
  % maxcitenames=1,
]{biblatex}
\renewcommand*{\mkbibnamegiven}[1]{%
  \ifitemannotation{highlight}%
  {\textbf{#1}}%
  {#1}}%
\renewcommand*{\mkbibnamefamily}[1]{%
  \ifitemannotation{highlight}%
  {\textbf{#1}}%
  {#1}%
  \ifitemannotation{first}%
  {\textsuperscript{*}}%
  {}%
  \ifitemannotation{corresponding}%
  {$^\dagger$}%
  {}%
}%%

\addbibresource{bibliography/authored/latentcommunication.bib}
\addbibresource{bibliography/authored/other.bib}
\addbibresource{bibliography/bibliography.bib} % The filename of the bibliography

% Force fullcite to use the full list of authors
\preto\fullcite{\AtNextCite{\defcounter{maxnames}{99}}}


==> glossaries/abbreviations.tex <==
% Possible abbreviations categories:
% - withdesc: with description, should be in fluent English
% - nolong: no long form in text, it has a description that should be in fluent English.
% - withoutdesc: without description, only short and long form

\newabbreviation[category=withoutdesc, sort=rsa]{rsa}{RSA}{Representational Similarity Analysis}


\newabbreviation[category=withoutdesc, sort=llm]{llm}{LLM}{Large Language Model}

\newabbreviation[category=withoutdesc, sort=wvlp]{wvlp}{WVLP}{Weakly Supervised Vision-and-Language Pretraining}

\newabbreviation[category=withoutdesc, sort=rlsa]{rlsa}{RLSA}{Relative Latent Space Aggregation}

\newabbreviation[category=withoutdesc, sort=ica]{ica}{ICA}{Independent Component Analysis}

\newabbreviation[category=withoutdesc, sort=ima]{ima}{IMA}{Independent Mechanism Analysis}

\newabbreviation[category=withoutdesc, sort=rl]{rl}{RL}{Reinforcement Learning}

\newabbreviation[category=withoutdesc, sort=pca]{pca}{PCA}{Principal Component Analysis}

\newabbreviation[category=withoutdesc, sort=qkv]{qkv}{QKV}{Query, Key, Value}

\newabbreviation[category=withoutdesc, sort=mlp]{mlp}{MLP}{Multi-Layer Perceptron}

\newabbreviation[category=withdesc, sort=svm, description={A Support Vector Machine (SVM) is a supervised learning model used for classification and regression tasks. It effectively creates a hyperplane or set of hyperplanes in a high-dimensional space, which can be used for classification, regression, or other tasks like outliers detection.}]{svm}{SVM}{Support Vector Machine}

\newabbreviation[category=withoutdesc, sort=cnn]{cnn}{CNN}{Convolutional Neural Network}

\newabbreviation[category=withoutdesc, sort=gnn]{gnn}{GNN}{Graph Neural Network}

\newabbreviation[category=withoutdesc, sort=linae]{linae}{LinAE}{Linearized AutoEncoder}

\newabbreviation[category=withoutdesc, sort=linvae]{linvae}{LinVAE}{Linearized Variational AutoEncoder}

\newabbreviation[category=withoutdesc, sort=vit]{vit}{ViT}{Vision Transformer}

\newabbreviation[category=withoutdesc, sort=ae]{ae}{AE}{AutoEncoder}

\newabbreviation[category=withoutdesc, sort=vae]{vae}{VAE}{Variational AutoEncoder}

\newabbreviation[category=withoutdesc, sort=relative]{rr}{RR}{Relative Representation}

\newabbreviation[category=withoutdesc, sort=rae]{rae}{RelAE}{Relative AutoEncoder}

\newabbreviation[category=withoutdesc, sort=rvae]{rvae}{RelVAE}{Relative Variational AutoEncoder}

\newabbreviation[category=withoutdesc, sort=ao]{ao}{AO}{Anchor Optimization}

\newabbreviation[category=withoutdesc, sort=mse]{mse}{MSE}{Mean Squared Error}

\newabbreviation[category=withoutdesc, sort=mae]{mae}{MAE}{Mean Absolute Error}

\newabbreviation[category=withoutdesc, sort=nn]{nn}{NN}{Neural Network}

\newabbreviation[category=withoutdesc, sort=nlp]{nlp}{NLP}{Natural Language Processing}

\newabbreviation[category=withoutdesc, sort=cv]{cv}{CV}{Computer Vision}

\newabbreviation[category=withoutdesc, sort=cka]{cka}{CKA}{Centered Kernel Alignment}

\newabbreviation[category=withoutdesc, sort=cca]{cca}{CCA}{Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=svcca]{svcca}{SVCCA}{Singular Value Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=pwcca]{pwcca}{PWCCA}{Projection Weighted Canonical Correlation Analysis}

\newabbreviation[category=withoutdesc, sort=svd]{svd}{SVD}{Singular Value Decomposition}

\newabbreviation[category=withoutdesc, sort=abs]{abs}{Abs.}{Absolute}

\newabbreviation[category=withoutdesc, sort=cos]{cos}{Cos.}{Cosine}

\newabbreviation[category=withoutdesc, sort=eu]{eu}{Eucl.}{Euclidean}

\newabbreviation[category=withoutdesc, sort=geo]{geo}{Geod.}{Geodesic}

\newabbreviation[category=withoutdesc, sort=at]{at}{AT}{Affine Transformation}

\newabbreviation[category=withoutdesc, sort=tr]{tr}{TR}{Translation}

\newabbreviation[category=withoutdesc, sort=lt]{lt}{LT}{Linear Transformation}

\newabbreviation[category=withoutdesc, sort=is]{is}{IS}{Isotropic Scaling}

\newabbreviation[category=withoutdesc, sort=ot]{ot}{OT}{Orthogonal Transformation}

\newabbreviation[category=withoutdesc, sort=pt]{pt}{PT}{Permutation}

\newabbreviation[category=withoutdesc, sort=mis]{mis}{MIS}{Manifold Isometry}

\newabbreviation[category=withdesc, sort=lcp, description={
            The Latent Communication Problem or Latent Space Communication Problem is a novel formalization of a problem arising in machine learning, specifically within the context of neural networks. The problem focuses on unifying semantically related manifolds embedded in different data spaces.
        }]{lcp}{LCP}{Latent Communication Problem}

\newabbreviation[category=nolong, description={The FastText word embeddings, a powerful model designed for text representation and classification \citep{bojanowski2016enriching}.}, sort=fasttext]{fasttext}{\texttt{FastText}}{\texttt{FastText}}

\newabbreviation[category=nolong, description={The Word2Vec word embeddings, renowned for transforming words into high-dimensional vector spaces, facilitating semantic analysis \citep{word2vec}.}, sort=word2vec]{word2vec}{\texttt{Word2Vec}}{\texttt{Word2Vec}}

\newabbreviation[category=nolong, description={The MNIST dataset  \citep{mnist}, a classic collection of handwritten digits widely used for training image processing systems.}, sort=mnist]{mnist}{\texttt{MNIST}}{\texttt{MNIST}}

\newabbreviation[category=withdesc, description={The Colored MNIST dataset \citep{Arjovsky2019-ig}, a variation of the original MNIST, incorporates color as an additional feature, challenging models to learn from both shape and color.}, sort=cmnist]{cmnist}{\texttt{C-MNIST}}{\texttt{Colored MNIST}}

\newabbreviation[category=withdesc, description={The Fashion MNIST dataset \citep{Xiao2017-er}, designed as a more complex alternative to the original MNIST, contains grayscale images of various fashion products.}, sort=fmnist]{fmnist}{\texttt{F-MNIST}}{\texttt{Fashion MNIST}}

\newabbreviation[category=nolong, description={The CIFAR-10 dataset \citep{Krizhevsky2009-hv}, composed of 60,000 32x32 color images in 10 classes, with 6,000 images per class.}, sort=cifart]{cifart}{\texttt{CIFAR-10}}{\texttt{CIFAR-10}}

\newabbreviation[category=nolong, description={The CIFAR-100 dataset \citep{Krizhevsky2009-hv}, similar to CIFAR-10 but with 100 classes, providing a more challenging task for image classification models.}, sort=cifarh]{cifarh}{\texttt{CIFAR-100}}{\texttt{CIFAR-100}}

\newabbreviation[category=nolong, description={The ImageNet1k dataset \citep{imagenet}, a large-scale dataset designed for use in visual object recognition software research.}, sort=imagenet1k]{imagenet1k}{\texttt{ImageNet1k}}{\texttt{ImageNet1k}}

\newabbreviation[category=withdesc, description={The ShapeNet dataset \citep{Chang2015-vc}, a collaborative effort to establish a richly-annotated, large-scale dataset of 3D shapes.}, sort=shapenet]{shapenet}{\texttt{ShapeNet}}{\texttt{ShapeNet}}

\newabbreviation[category=withdesc, description={The FAUST dataset \citep{Bogo2014-bh}, a collection of high-resolution 3D scans of human figures, designed to support research in computer vision and graphics.}, sort=faust]{faust}{\texttt{FAUST}}{\texttt{FAUST}}

\newabbreviation[category=withdesc, description={The COMA dataset \citep{Ranjan2018-zx}, consisting of 3D facial expressions, captured from a variety of subjects, to facilitate research in dynamic facial expression analysis.}, sort=coma]{coma}{\texttt{COMA}}{\texttt{COMA}}

\newabbreviation[category=nolong, description={The Amazon Reviews dataset \citep{amazon-reviews}, a large collection of customer reviews, useful for sentiment analysis and other forms of Natural Language Processing.}, sort=amazon]{amazon}{\texttt{Amazon Reviews}}{\texttt{Amazon Reviews}}

\newabbreviation[category=nolong, description={The AG News dataset \citep{Zhang2015CharacterlevelCN}, a collection of news articles for use in Natural Language Processing tasks such as text classification and sentiment analysis.}, sort=agnews]{agnews}{\texttt{AG News}}{\texttt{AG News}}

\newabbreviation[category=nolong, description={The DBpedia dataset \citep{Auer2007-fb}, derived from Wikipedia, provides a structured form of Wikipedia's content for various knowledge extraction and semantic search tasks.}, sort=dbpedia]{dbpedia}{\texttt{DBpedia}}{\texttt{DBpedia}}

\newabbreviation[category=nolong, description={The IMDB dataset \citep{imdb}, a set of movie reviews for binary sentiment classification, widely used in Natural Language Processing research.}, sort=imdb]{imdb}{\texttt{IMDB}}{\texttt{IMDB}}

\newabbreviation[category=nolong, description={The N24News dataset \citep{n24news}, a collection of news articles with associated images.}, sort=n24news]{n24news}{\texttt{N24News}}{\texttt{N24News}}

\newabbreviation[category=nolong, description={The TREC dataset \citep{trec,li-roth-2002-learning}, designed for research in text retrieval and information extraction, includes a wide range of question types.}, sort=trec]{trec}{\texttt{TREC}}{\texttt{TREC}}

\newabbreviation[category=nolong, description={The Cora dataset \citep{corapubmed}, a collection of scientific publications categorized into different classes, used for document classification and citation prediction.}, sort=cora]{cora}{\texttt{Cora}}{\texttt{Cora}}

\newabbreviation[category=nolong, description={The CiteSeer dataset \citep{citeseer}, an academic literature digital library and search engine that focuses primarily on the literature in computer and information science.}, sort=citeseer]{citeseer}{\texttt{CiteSeer}}{\texttt{CiteSeer}}

\newabbreviation[category=nolong, description={The PubMed dataset \citep{corapubmed}, comprising abstracts from biomedical literature, serves as a resource for tasks like biomedical entity recognition and relation extraction.}, sort=pubmed]{pubmed}{\texttt{PubMed}}{\texttt{PubMed}}

\newabbreviation[category=withdesc, description={The Thingi10K dataset \citep{Zhou_undated-jc}, an extensive collection of 3D printing models, provides a diverse set of shapes for tasks like 3D object recognition and segmentation.}, sort=thingi]{thingi}{\texttt{Thingi10K}}{\texttt{Thingi10K}}

\newabbreviation[category=withdesc, description={The SURREAL dataset \citep{Varol2017-et}, containing synthetic images of humans in various poses and clothing, aims to support the development of models that can understand human body dynamics.}, sort=surreal]{surreal}{\texttt{SURREAL}}{\texttt{SURREAL}}

\newabbreviation[category=withdesc, description={The DeformingThings4D dataset \citep{Niesner_undated-ny}, a collection of 4D scans that capture the dynamic deformation of objects, is invaluable for understanding temporal changes in shape.}, sort=deformingthings]{deformingthings}{\texttt{DeformingThings4D}}{\texttt{DeformingThings4D}}

\newabbreviation[category=withdesc, description={The BERT model \citep{bert} with a base configuration and cased vocabulary, a breakthrough in the field of Natural Language Processing. Available pre-trained on HuggingFace.}, sort=bertbc]{bertbc}{BERT-C}{\texttt{bert-base-cased}}

\newabbreviation[category=withdesc, description={The BERT model \citep{bert} with a base configuration and uncased vocabulary, providing a foundational architecture for developing advanced Natural Language Processing systems. Available pre-trained on HuggingFace}, sort=bertbu]{bertbu}{BERT-U}{\texttt{bert-base-uncased}}

\newabbreviation[category=withdesc, description={The ELECTRA model \citep{electra} with a base discriminator configuration, introducing a novel pre-training methodology for language representations that is both efficient and effective. Available pre-trained on HuggingFace}, sort=electrabd]{electrabd}{ELECTRA}{\texttt{google/electra-base-discriminator}}

\newabbreviation[category=withdesc, description={The RoBERTa model \citep{roberta} with a base configuration, an optimized version of BERT that improves language understanding by carefully tuning hyperparameters and training with more data. Available pre-trained on HuggingFace}, sort=robertab]{robertab}{RoBERTa}{\texttt{roberta-base}}

\newabbreviation[category=withdesc, description={The ALBERT model \citep{albert} with a base version 2 configuration, a lighter and more efficient version of BERT, designed to reduce model size while maintaining performance. Available pre-trained on HuggingFace}, sort=albertbv2]{albertbv2}{ALBERT}{\texttt{albert-base-v2}}

\newabbreviation[category=withdesc, description={The XLM-RoBERTa model  \citep{xlmr} with a base configuration, extends the RoBERTa architecture to support multilingual language processing, enabling improved cross-lingual performance. Available pre-trained on HuggingFace}, sort=xlmrobertab]{xlmrobertab}{XLM-R}{\texttt{xlm-roberta-base}}

\newabbreviation[category=withdesc, description={The CLIP model \citep{clip} with a ViT-base and patch32 configuration, a state-of-the-art model for connecting visual and textual data, facilitating robust image-text understanding. Available pre-trained on HuggingFace}, sort=clip]{clip}{CLIP}{\texttt{openai/clip-vit-base-patch32}}

\newabbreviation[category=withdesc, description={The RexNet model \citep{rexnet} with 100 layers, exemplifies the advances in neural network architecture for efficient and effective image processing. Available pre-trained on HuggingFace}, sort=rexnet100]{rexnet100}{RexNet}{\texttt{rexnet\_100}}

\newabbreviation[category=withdesc, description={The CSPDarkNet53 architecture, represents a significant advancement in the field of computer vision, offering a robust backbone for object detection models. Available pre-trained on HuggingFace}, sort=cspdarknet53]{cspdarknet53}{DarkNet}{\texttt{cspdarknet53}}

\newabbreviation[category=withdesc, description={The ViT model \citep{vit} with a small configuration, patch size 16, and image size 224, introduces a novel approach to image classification, leveraging transformer architecture for visual tasks. Available pre-trained on HuggingFace}, sort=vitsp16224]{vitsp16224}{ViT-S/16}{\texttt{vit\_small\_patch16\_224}}

\newabbreviation[category=withdesc, description={The ViT model \citep{vit} with a base configuration, patch size 16, and image size 224, introduces a novel approach to image classification, leveraging transformer architecture for visual tasks. Available pre-trained on HuggingFace}, sort=vitbp16224]{vitbp16224}{ViT-B/16}{\texttt{vit\_base\_patch16\_224}}

\newabbreviation[category=withdesc, description={The ViT model \citep{vit} with a base configuration, patch size 16, and image size 384, introduces a novel approach to image classification, leveraging transformer architecture for visual tasks. Available pre-trained on HuggingFace}, sort=vitbp16384]{vitbp16384}{ViT-B/16L}{\texttt{vit\_base\_patch16\_384}}

\newabbreviation[category=withdesc, description={The ViT model \citep{vit} with a base configuration, the ResNet50 backbone, and image size 384, combines the strengths of convolutional neural networks and transformer models for superior image analysis capabilities. Available pre-trained on HuggingFace}, sort=vitbr50384]{vitbr50384}{RViT-B/16}{\texttt{vit\_base\_resnet50\_384}}


==> glossaries/symbols.tex <==
\glsxtrnewsymbol[sort=rp, description={The relative projection function calculates the representations of a point \gls{zx} relative to a set of anchor points \gls{ZA}, utilizing the similarity function \gls{sim}.}]{relativeprojection}{\ensuremath{R_p}}

\glsxtrnewsymbol[sort=p, description={This function aggregates the relative spaces formed by different similarity functions \gls{sim}, for instance, through concatenation.}]{aggregation}{\ensuremath{\rho}}

\glsxtrnewsymbol[sort=A, description={Represents a subset of the training data \gls{X} or \gls{Y}, denoted as anchor samples.}]{anchors}{\ensuremath{A}}

\glsxtrnewsymbol[sort=AZ, description={The anchors embeddings, derived from the anchors \gls{anchors} through an encoding process.}]{ZA}{\ensuremath{\widetilde{\gls{anchors}}}}

\glsxtrnewsymbol[sort=a, description={Denotes a particular anchor point within \gls{anchors}.}]{a}{\ensuremath{{a}}}

\glsxtrnewsymbol[sort=az, description={A specific anchor point from \gls{anchors}, encoded into a latent space by \gls{enc}.}]{za}{\ensuremath{\widetilde{a}}}

\glsxtrnewsymbol[sort=sim, description={Aa generic function that assesses similarity between two latent representations.}]{sim}{\ensuremath{d}}

\glsxtrnewsymbol[sort=s, description={The similarity score obtained through the generic similarity function \gls{sim}.}]{simscore}{\ensuremath{s}}

\glsxtrnewsymbol[sort=r, description={Represents the relative representation of \gls{x} with respect to certain anchors \gls{anchors}.}]{r}{\ensuremath{r}}

\glsxtrnewsymbol[sort=Ap, description={Anchor samples drawn simultaneously from both domains \gls{X} and \gls{Y}, denoted as parallel anchors, forming a subset of \gls{pi}.}]{parallelanchors}{\ensuremath{\gls{anchors}_{\gls{X}\gls{Y}}}}

\glsxtrnewsymbol[sort=ApS, description={A small subset of parallel anchors \gls{parallelanchors}, i.e. $|\gls{parallelseeds}| \ll |\gls{parallelanchors}|$}]{parallelseeds}{\ensuremath{\gls{seeds}_{\gls{X}\gls{Y}}}}

\glsxtrnewsymbol[sort=AS, description={A small subset of anchors \gls{anchors}, i.e. $|\gls{seeds}| \ll |\gls{anchors}|$}]{seeds}{\ensuremath{\Lambda}}

\glsxtrnewsymbol[sort=ApSZ, description={A small subset of parallel anchors \gls{parallelanchors} embedded in a latent space through some encoding process}]{zparallelseeds}{\ensuremath{\widetilde{\gls{seeds}}_{\gls{X}\gls{Y}}}}

\glsxtrnewsymbol[sort=ASZ, description={A small subset of anchors \gls{anchors} embedded in a latent space through some encoding process}]{zseeds}{\ensuremath{\widetilde{\gls{seeds}}}}

\glsxtrnewsymbol[sort=AOOD, description={Out-of-domain anchors, i.e., anchors chosen from a domain different from the training distribution. Used to construct relative representations in domain adaptation tasks with limited correspondence and labeled data.}]{OODanchors}{\ensuremath{\widehat{\gls{anchors}}}}

\glsxtrnewsymbol[sort=S, description={A generic space, potentially an input, latent, or any conceptual space where data or representations are defined.}]{S}{\ensuremath{{S}}}

\glsxtrnewsymbol[sort=s, description={An element within the generic space \gls{S}.}]{s}{\ensuremath{s}}

\glsxtrnewsymbol[sort=C, description={An abstract semantic link between abstract data manifolds \gls{Mx} and \gls{My}, critical for understanding semantic alignment between different data representations, though not directly observable.}]{C}{\ensuremath{\mathcal{C}}}

\glsxtrnewsymbol[sort=pi, description={Observable pairs from \gls{X} and \gls{Y} that are semantically connected, derived from the theoretical correspondence \gls{C}.}]{pi}{\ensuremath{\pi}}

\glsxtrnewsymbol[sort=Rd, description={A Euclidean space with $d$ dimensions.}]{Rd}{\ensuremath{\mathbb{R}^d}}

\glsxtrnewsymbol[sort=R, description={Denotes the set of all real numbers.}]{R}{\ensuremath{\mathbb{R}}}

\glsxtrnewsymbol[sort=phi, description={A collection of factors, including weight initialization, data shuffling, hyperparameters, and other stochastic factors, that collectively affect the training dynamics of neural networks, influencing the learned latent spaces.}]{randomfactors}{\ensuremath{\phi}}

\glsxtrnewsymbol[sort=transformation, description={A transformation induced by changing the factors $\gls{randomfactors}$ over the latent space.}]{transformation}{\ensuremath{\mathcal{T}}}

\glsxtrnewsymbol[sort=transformationapprox, description={An estimate of the transformation between latent spaces, induced by changes in $\gls{randomfactors}$.}]{transformationapprox}{\ensuremath{\widehat{\mathcal{T}}}}

\glsxtrnewsymbol[sort=transformationclass, description={An unknown class of transformations that the induced transformation $\gls{transformation}$ belongs to. It depends on the data distribution, the task, additional contraints on the network, and possibly other factors.}]{transformationclass}{\ensuremath{\mathbb{T}}}

\glsxtrnewsymbol[sort=E, description={The expectation operator, representing the average value of a random variable over a given distribution.}]{expectation}{\ensuremath{\mathbb{E}}}

\glsxtrnewsymbol[sort=Reg, description={A function that encodes additional constraints on the weights \gls{theta}.}]{Reg}{\ensuremath{Reg}}

\glsxtrnewsymbol[sort=Z, description={The input space associated with domain Z, similar to \gls{X} but for a potentially different type of data or domain.}]{Z}{{\ensuremath{{Z}}}}

\glsxtrnewsymbol[sort=X, description={The input space associated with domain X, encompassing all possible inputs that can be processed or generated within this context.}]{X}{\textcolor{colorxstuff}{\ensuremath{{X}}}}

\glsxtrnewsymbol[sort=Y, description={The input space associated with domain Y, similar to \gls{X} but for a potentially different data modality or domain.}]{Y}{\textcolor{colorystuff}{\ensuremath{{Y}}}}

\glsxtrnewsymbol[sort=x, description={A data point or sample from the input space \gls{X}, representing an instance in this domain.}]{x}{\textcolor{colorxstuff}{\ensuremath{{x}}}}

\glsxtrnewsymbol[sort=y, description={A data point or sample from the input space \gls{Y}, akin to \gls{x} but from domain \gls{Y}.}]{y}{\textcolor{colorystuff}{\ensuremath{{y}}}}

\glsxtrnewsymbol[sort=M, description={An abstract manifold representing the semantic of some data.}]{M}{\ensuremath{\mathcal{M}}}

\glsxtrnewsymbol[sort=Mx, description={The manifold for input space \gls{X}, encapsulating the data underlying meaning in this domain.}]{Mx}{\textcolor{colorxstuff}{\ensuremath{\mathcal{M}_{\gls{X}}}}}

\glsxtrnewsymbol[sort=My, description={The manifold for input space \gls{Y}, analogous to \gls{Mx} but for domain \gls{Y}.}]{My}{\textcolor{colorystuff}{\ensuremath{\mathcal{M}_{\gls{Y}}}}}

\glsxtrnewsymbol[sort=xm, description={A point on the manifold \gls{Mx}.}]{mx}{\textcolor{colorxstuff}{\ensuremath{\mathscr{x}}}}

\glsxtrnewsymbol[sort=ym, description={A point on the manifold \gls{My}, akin to \gls{mx} but for domain \gls{Y}.}]{my}{\textcolor{colorystuff}{\ensuremath{\mathscr{y}}}}

\glsxtrnewsymbol[sort=XZ, description={The latent space derived from input space \gls{X}, representing encoded data.}]{ZX}{\textcolor{colorxstuff}{\ensuremath{\widetilde{X}}}}

\glsxtrnewsymbol[sort=YZ, description={The latent space derived from input space \gls{Y}, analogous to \gls{ZX} but for domain \gls{Y}.}]{ZY}{\textcolor{colorystuff}{\ensuremath{\widetilde{Y}}}}

\glsxtrnewsymbol[sort=yz, description={A sample in the latent space \gls{ZY}, encoded from an input in \gls{Y}.}]{zy}{\textcolor{colorystuff}{\ensuremath{\widetilde{y}}}}

\glsxtrnewsymbol[sort=xz, description={A sample in the latent space \gls{ZX}, encoded from an input in \gls{X}.}]{zx}{\textcolor{colorxstuff}{\ensuremath{\widetilde{x}}}}

\glsxtrnewsymbol[sort=MZ, description={An abstract manifold associated with a latent space, representing the semantic of data in its encoded form.}]{ZM}{\ensuremath{\widetilde{{\mathcal{M}}}}}

\glsxtrnewsymbol[sort=MxZ, description={The latent manifold associated with the latent space \gls{ZX}, representing the underlying meaning of encoded data from \gls{X}.}]{ZMx}{\textcolor{colorxstuff}{\ensuremath{\widetilde{{\mathcal{M}}}_{\gls{X}}}}}

\glsxtrnewsymbol[sort=MyZ, description={The latent manifold for space \gls{ZY}, similar to \gls{ZMx} but for encoded data from \gls{Y}.}]{ZMy}{\textcolor{colorystuff}{\ensuremath{\widetilde{{\mathcal{M}}}_{\gls{Y}}}}}

\glsxtrnewsymbol[sort=xzm, description={A point on the latent manifold \gls{ZMx}.}]{zmx}{\textcolor{colorxstuff}{\ensuremath{\widetilde{{\mathscr{x}}}}}}

\glsxtrnewsymbol[sort=yzm, description={A point on the latent manifold \gls{ZMy}, similar to \gls{zmx}.}]{zmy}{\textcolor{colorystuff}{\ensuremath{\widetilde{{\mathscr{y}}}}}}


\glsxtrnewsymbol[sort=Tx, description={A transformation applied to data in the latent space $\gls{Tx}: \gls{ZX} \to \gls{UX}$, used for unifying or translating between latent spaces.}]{Tx}{\textcolor{colorxstuff}{\ensuremath{T_{\gls{X}}}}}

\glsxtrnewsymbol[sort=Ty, description={A transformation applied to data in space $\gls{Ty}: \gls{ZY} \to \gls{UY}$, similar to \gls{Tx} but for domain \gls{Y}.}]{Ty}{\textcolor{colorystuff}{\ensuremath{T_{\gls{Y}}}}}

\glsxtrnewsymbol[sort=U, description={A universal space that includes the spaces \gls{UX} and \gls{UY}, where latent manifold embeddings coincide for both \gls{X} and \gls{Y}.}]{U}{\ensuremath{U}}

\glsxtrnewsymbol[sort=UX, description={A universal space into which \gls{X} (and their latent representations) can be mapped.}]{UX}{\textcolor{colorxstuff}{\ensuremath{U_{\gls{X}}}}}

\glsxtrnewsymbol[sort=UY, description={A universal space similar to \gls{UX}, but dedicated to the domain \gls{Y}.}]{UY}{\textcolor{colorystuff}{\ensuremath{U_{\gls{Y}}}}}

\glsxtrnewsymbol[sort=up, description={A product space of invariant components approximating \gls{U}, a universal space including \gls{UX} and \gls{UY} with identical latent manifold embeddings for both domains.}]{productspace}{\ensuremath{\widehat{\gls{U}}}}


\glsxtrnewsymbol[sort=NN, description={A general neural network architecture, described as combining encoder and decoder functions: $\gls{dec}\circ\gls{enc}$, capable of representing complex functions through layers of interconnected neurons.}]{N}{\ensuremath{N}}

\glsxtrnewsymbol[sort=enc, description={The neural network's encoding function, converting input data into a latent representation.}]{enc}{\ensuremath{E}}

\glsxtrnewsymbol[sort=dec, description={The neural network's decoding function, responsible to \gls{task}, such as data classification or reconstruction.}]{dec}{\ensuremath{D}}

\glsxtrnewsymbol[sort=Dall, description={The set of all possible decoder architectures and their parameterizations that can be employed to solve a specific task, representing the space of solutions in the context of neural network design.}]{Dall}{\ensuremath{\mathbb{D}}}

\glsxtrnewsymbol[sort=task, description={A specific problem addressed by neural networks, including classification, regression, and data generation, among others.}]{task}{\ensuremath{\mathsf{T}}}

\glsxtrnewsymbol[sort=loss, description={The function measuring a neural network's performance on a specified task \gls{task}.}]{loss}{\ensuremath{\mathcal{L}}}

\glsxtrnewsymbol[sort=theta, description={The neural network's parameters, such as weights and biases, adjusted during training to minimize the loss function.}]{theta}{\ensuremath{\theta}}

\glsxtrnewsymbol[sort=phiX, description={The embedding function mapping data points from the data manifold \gls{Mx} to the input space \gls{X}, representing how abstract, low-dimensional structures are realized within the high-dimensional space.}]{phiX}{\textcolor{colorxstuff}{\ensuremath{\varphi_{\gls{X}}}}}

\glsxtrnewsymbol[sort=phiY, description={The embedding function mapping data points from the data manifold \gls{My} to the input space \gls{Y}, analogous to \gls{phiX} but specific to the domain \gls{Y}.}]{phiY}{\textcolor{colorystuff}{\ensuremath{\varphi_{\gls{Y}}}}}

\glsxtrnewsymbol[sort=phiZX, description={The embedding function mapping data points from the latent data manifold \gls{ZMx} to the latent space \gls{ZX}, representing how encoded, abstract structures are realized within the latent high-dimensional space \gls{ZX}.}]{phiZX}{\textcolor{colorxstuff}{\ensuremath{\varphi_{\gls{ZX}}}}}

\glsxtrnewsymbol[sort=phiZY, description={The embedding function mapping data points from the latent data manifold \gls{ZMy} to the latent space \gls{ZY}, analogous to \gls{phiZX} but specific to the domain \gls{Y}.}]{phiZY}{\textcolor{colorystuff}{\ensuremath{\varphi_{\gls{ZY}}}}}

\glsxtrnewsymbol[sort=phi, description={A embedding function, in the mathematical sense, that maps data points from a manifold \gls{M} to a space \gls{S}, encapsulating the concept of manifold learning and data representation.}]{phi}{\ensuremath{\varphi}}

\glsxtrnewsymbol[sort=l1, description={Represents the Manhattan distance metric.}]{l1}{$L_1$}

\glsxtrnewsymbol[sort=linf, description={Denotes the Chebyshev distance metric.}]{linf}{$L_{\infty}$}

